Compositional Algorithms on Compositional Data: Deciding Sheaves on Presheaves

Algorithmicists are well-aware that fast dynamic programming algorithms are very often the correct choice when computing on compositional (or even recursive) graphs. Here we initiate the study of how to generalize this folklore intuition to mathematical structures writ large. We achieve this horizontal generality by adopting a categorial perspective which allows us to show that: (1) structured decompositions (a recent, abstract generalization of many graph decompositions) define Grothendieck topologies on categories of data (adhesive categories) and that (2) any computational problem which can be represented as a sheaf with respect to these topologies can be decided in linear time on classes of inputs which admit decompositions of bounded width and whose decomposition shapes have bounded feedback vertex number. This immediately leads to algorithms on objects of any C-set category; these include -- to name but a few examples -- structures such as: symmetric graphs, directed graphs, directed multigraphs, hypergraphs, directed hypergraphs, databases, simplicial complexes, circular port graphs and half-edge graphs. Thus we initiate the bridging of tools from sheaf theory, structural graph theory and parameterized complexity theory; we believe this to be a very fruitful approach for a general, algebraic theory of dynamic programming algorithms. Finally we pair our theoretical results with concrete implementations of our main algorithmic contribution in the AlgebraicJulia ecosystem.

==> SheafTopImplication.tex <==
In the general case, there are going to be many distinct Grothendieck topologies that we could attach to a particular category, yielding different sites. In building a particular site, we have in mind the sheaves that will be defined with respect to it. It would be nice if we could use some relationship between sites to induce a relationship between the associated sheaves, and reduce our work by lifting the computation of sheaves with respect to one Grothendieck topology from the sheaves on another (appropriately related) Grothendieck topology. As it turns out, the collection of Grothendieck topologies on a category $\textbf{C}$ are partially ordered (by inclusion), and established results show us how to exploit this to push sheaves on one topology to sheaves on others. \par 
	We might first define maps between arbitrary coverings as follows: 
	\begin{definition}
		\normalfont 
		A \textbf{morphism of coverings} from $\mathcal{V} = \{V_j \rightarrow V\}_{j \in J}$ to $\mathcal{U} = \{U_i \rightarrow U\}_{i \in I}$ is an arrow $V \rightarrow U$ together with a pair $(\sigma, f)$ comprised of 
		\begin{itemize}
			\item a function $\sigma: J \rightarrow I$ on the index sets, and 
			\item a collection of morphisms $f = \{f_j: V_j \rightarrow U_{\sigma(j)}\}_{j \in J}$ with 
			\begin{center}
				\begin{tikzcd}
					V_j \arrow[d] \arrow[r] & U_{\sigma(j)} \arrow[d] \\ 
					V \arrow[r] & U
				\end{tikzcd}
			\end{center}
			commuting for all $j \in J$.
		\end{itemize}
	\end{definition}
	With this notion of morphisms, we could define a category of the coverings on $\textbf{C}$. However, we will mostly be concerned with a particular case of such morphisms of coverings, namely where $V = U$ and $V \rightarrow U$ is just the identity map. In this case, we say that $\mathcal{V}$ is a \textbf{refinement} of $\mathcal{U}$.
	\begin{definition}
		\normalfont 
		$\textbf{C}$ a category, $\mathcal{U} = \{U_i \rightarrow U\}_{i \in I}$ a family of arrows. Then a \textbf{refinement} $\mathcal{V} = \{V_j \rightarrow U\}_{j \in J}$ is a family of arrows such that for each index $j \in J$ there exists some $i \in I$ such that $V_j \rightarrow U$ factors through $U_i \rightarrow U$.
	\end{definition}
	In sieve terms, we can simplify the above to say that, given $\mathcal{U} = \{U_i \rightarrow U\}$ and $\mathcal{V} = \{V_j \rightarrow U\}$, $\mathcal{V}$ is a refinement of $\mathcal{U}$ iff the sieve generated by $\mathcal{V}$ is contained in (a sub-sieve of) the sieve generated by $\mathcal{U}$. \par 
	Moreover, observe that any covering is a refinement of itself, and a refinement of a refinement is a refinement. As such, refinement gives us an ordering on the coverings of an object $U$. We can use this to define the following relation for Grothendieck topologies. 
	\begin{definition}
		\normalfont 
		 Let $\textbf{C}$ be a category and $J, J'$ two Grothendieck topologies on $\textbf{C}$. We say that $J$ is \textbf{subordinate to} $J'$, denoted $J \leqslant J'$, provided every covering in $J$ has a refinement that is a covering in $J'$. \par 
		 If $J \leqslant J'$ and $J' \leqslant J$, then $J$ and $J'$ are \textbf{equivalent}.
	\end{definition}
	This really says not just that any covering in $J$ is a covering in $J'$---which makes us say that the topology $J'$ is finer than $J$---but that for any covering in $J$, there exists a refinement among the coverings in $J'$. \par 
	In sieve terms, $J \leqslant J'$ just says that for any object $U$ and any sieve $S$ considered a covering sieve by $J$, there exists a sieve $S'$ that is considered a covering sieve by $J'$, where all arrows of $S$ are also in $S'$. In particular, two topologies will be equivalent iff they have the same sieves. \par 
Now we come to the point of these definitions. Using the main sheaf definition---i.e., a functor $F$ is a sheaf with respect to a topology $J$ iff for any sieve $S$ belonging to $J$ the induced map 
\begin{equation*}
F(U) \simeq \text{Hom}(Y_U, F) \rightarrow \text{Hom}(S, F)
\end{equation*}
is a bijection---together with the previous definition (expressed in terms of sieves), we get the following result.
	\begin{proposition} \label{MainResult}
		Let $J, J'$ be two Grothendieck topologies on the same category $\textbf{C}$. If $J$ is  subordinate to $J'$, i.e., $J \leqslant J'$, then every presheaf that satisfies the sheaf condition for $J'$ also satisfies it for $J$.
	\end{proposition}
	In other words: if $J$ is subordinate to $J'$, then we know that any sheaf for $J'$ will automatically be a sheaf for $J$. 
	\begin{proof} 
		We could show the result by deploying the notion of morphisms of sites (see nLab) $f: (\textbf{C}, J) \rightarrow (\textbf{D}, K)$, as a certain ``cover-preserving" morphism, where this is got by setting $\textbf{D} = \textbf{C}$ and $K = J'$, and using the identity functor $\textbf{C} \rightarrow \textbf{C}$, taking any object to itself and any $J$-covering to itself as well. Precomposition with $f$ gives a functor between the category of presheaves (going the other way), and we then use the pushforward (or direct image) functor $f_*: \textbf{Sh}(\textbf{C}, J') \rightarrow \textbf{Sh}(\textbf{C}, J)$, where this is the restriction of the precomposition with $f$ down to sheaves, to push a sheaf with respect to $J'$ to a sheaf $f_* F$ on $J$. Details can be found in the literature.
	\end{proof}
	As a particular case, two equivalent topologies have the same sheaves. \par 
	The main take-away here is, of course, that if we can show that a particular presheaf is in fact a sheaf with respect to a topology $J'$, and if $J$ is another topology which we can establish is subordinate to $J'$, then we will get for free a sheaf with respect to $J$ (and with respect to any other subordinate topology, for that matter). Moreover, in particular, if there is a \textit{finest} cover, verifying the sheaf axiom there will guarantee it for all covers. \par 
	Let's now connect these established results to the Grothendieck topologies that we define, namely monDiag and Dcmp, where the latter is a subfunctor of the former. We can focus on showing how $\text{monDiag}$ relates to another Grothendieck topology of interest.
	\begin{proposition}
		The topology given by $\text{monDiag}$ is subordinate to the subobject topology.
	\end{proposition}
	\begin{proof}
		The subobject topology just takes for coverings of an object $c$ (equivalence classes of) monomorphisms whose union is $c$. Need to show that any covering in the monic diagram topology can be refined by a covering in the subobject topology. Compare to the def of $\text{monDiag}$ in Cor 4.4.
	\end{proof}
	Provided this is true, using Proposition \ref{MainResult}, we have the following useful result.
	\begin{proposition} \normalfont 
		If a presheaf is a sheaf with respect to the subobject topology, then it will automatically give us a sheaf with respect to the monDiag (or decomp) topology. 
	\end{proposition}
